Exploring Hidden Dimensions in Parallelizing Convolutional Neural Networks

The past few years have witnessed growth in the computational requirements for training deep convolutional neural networks. Current approaches parallelize training onto multiple devices by applying a single parallelization strategy (e.g., data or model parallelism) to all layers in a network. Although easy to reason about, these approaches result in suboptimal runtime performance in large-scale distributed training, since different layers in a network may prefer different parallelization strategies. In this paper, we propose layer-wise parallelism that allows each layer in a network to use an individual parallelization strategy. We jointly optimize how each layer is parallelized by solving a graph search problem. Our evaluation shows that layer-wise parallelism outperforms state-of-the-art approaches by increasing training throughput, reducing communication costs, achieving better scalability to multiple GPUs, while maintaining original network accuracy.

==> impl.tex <==
\section{Implementation}
\label{sec:impl}
We found that it is non-trivial to parallelize the training of CNNs in the height, width, and channel dimensions
 in existing frameworks (e.g., \tensorflow, \pytorch, and \caffe), and none
 provides an interface for defining parallelism configurations for each layer.
We implemented our framework in Legion~\cite{Legion12}, a high-performance parallel runtime for
distributed heterogeneous architectures, and use cuDNN~\cite{cudnn} and cuBLAS~\cite{cublas}
as the underlying libraries for processing the layers in a network. 
The following Legion features significantly simplify our implementation.
First, Legion supports high-dimensional partitioning that allows us to parallelize any layer in any
combination of the dimensions. Second, Legion allows
to control parallelism at the granularity of each layer.
Third, Legion allows fine-grain control over the placement of data in memory. 
Fourth, Legion's asynchronous tasking model makes it easy to exploit task as well as image parallelism.
%We also include two critical optimizations that help achieve good performance.

%{\bf Overlapping computation with data transfers}.
%\Sys manages the gradients of each
%operation separately and transfers an operation's gradients as long as its back propagation is completed.
%We have found that this can effectively hide the data transfer overhead for gradient synchronization. As a result, the synchronous training performance matches
%asynchronous training in \Sys, which allows users to use synchronous training with its better algorithmic efficiency. 

%{\bf Distributing parameter servers}.
%Existing frameworks use {\em parameter servers} to store and update variables for a CNN model. Parameter servers are 
%located in CPU memory in \tensorflow and \pytorch. Because \Sys manages the parameters for
%each operation separately, \Sys can opportunistically distribute the parameter server onto the GPU memories 
%whenever possible. This eliminates data transfers for operations whose gradients and parameter server are located on the same GPU
%and transforms all GPU to CPU copies into faster GPU to GPU copies.


==> search.tex <==
\section{Finding Optimal Global Configurations}
\label{sec:search}

\begin{figure}[h]
\vspace{-5mm}
\begin{center}
\subfloat[Node elimination.]{
\includegraphics[scale=0.35]{figures/reduce_node.pdf}
\label{fig:reduce_node}
}
\subfloat[Edge elimination.]{
\includegraphics[scale=0.35]{figures/reduce_edge.pdf}
\label{fig:reduce_edge}
}
\caption{Performing a node/edge elimination on a computation graph.}
\end{center}
\vspace{-3mm}
\end{figure}

We now describe our algorithm for finding a global configuration that minimizes Equation~\ref{eqn1}.
In \Sys, each node can select any of a fixed (but large) set of parallelism configurations. Therefore the number of potential global
configurations is exponential in the number of nodes in a computation graph, which makes it impractical
to enumerate all global configurations for deep CNNs such as \vgg and \inception. 

However, the CNNs we have seen in practice exhibit strong locality: each node is only connected to a few
nodes with similar depth in a computation graph. Based on this observation, we use the following two elimination strategies to iteratively simplify the computation
graph while preserving the globally optimal configuration.

{\bf Node elimination}. For each node $w$ with a single in-edge $e_1=(u, w)$ and a single out-edge $e_2=(w, v)$, we remove node $w$ and the two edges
$e_1$ and $e_2$ from the graph and insert a new edge $e'=(u, v)$ (shown in Figure~\ref{fig:reduce_node}). The ${\er{xfer}()}$ function for node $e'$ is
\begin{equation}
\label{eqn2}
e'.{\er{xfer}}(c_u, c_v) = \min_{c_w} \{ e_1.{\er{xfer}}(c_u, c_w) + w.{\er{compute}}(c_w) + w.{\er{update}}(c_w) + e_2.{\er{xfer}}(c_w, c_v) \}
\end{equation}
Note that because we have precomputed the $\er{xfer}()$ function for edges in the original graph, we can similarly compute the $\er{xfer}()$ function for the transitive edge added by a node elimination;
 i.e., we use dynamic programming to compute the optimal configuration for node $w$ for every possible choice of configurations for nodes $u$ and $v$.
 For CNNs with a linear computation graph (e.g., \alexnet and \vgg), node elimination is sufficient to reduce the original graph to a graph with only 2 nodes.

{\bf Edge elimination}. For two edges with the same source and destination node (i.e., $e_1=(u, v)$ and $e_2=(u, v)$), we can remove $e_1$ and $e_2$ from
the graph and insert a new edge $e'=(u,v)$ (shown in Figure~\ref{fig:reduce_edge}). The ${\er{xfer}()}$ function for node $e'$ is
\begin{equation}
\label{eqn3}
e'.{\er{xfer}}(c_u, c_v) = e_1.{\er{xfer}}(c_u, c_v) + e_2.{\er{xfer}}(c_u, c_v)
\end{equation}

\begin{figure*}[h]
\vspace{-5mm}
\begin{center}
\subfloat[Initial computation graph.] {
\includegraphics[scale=0.25]{figures/sample1.pdf}
}
\subfloat[Node elimination.] {
\includegraphics[scale=0.25]{figures/sample2.pdf}
}
\subfloat[Edge elimination.] {
\includegraphics[scale=0.25]{figures/sample3.pdf}
}
\subfloat[Node elimination.] {
\includegraphics[scale=0.44]{figures/sample4.pdf}
}
\subfloat[Edge elimination.] {
\includegraphics[scale=0.44]{figures/sample5.pdf}
}
\caption{Iteratively performing node/edge eliminations on an Inception module.}
\label{fig:reduce_example}
\end{center}
\vspace{-3mm}
\end{figure*}

As with node elimination, we compute the $\er{xfer}()$ function for $e'$ using the already computed $\er{xfer}()$ functions for $e_1$ and $e_2$.
Figure~\ref{fig:reduce_example} shows how \Sys iteratively eliminates nodes and edges for an \inception module.
The full \inception computation graph has 120 nodes, which \Sys reduces to a 2-node graph.

\Sys iteratively uses node and edge eliminations to simplify a computation graph until neither elimination can be applied. \Sys then enumerates all
global configurations for the final graph and chooses the one that minimizes the $\er{Cost}$ function in Equation~\ref{eqn1}.

After deciding the configuration for each node in the final graph, \Sys then decides the configuration for the eliminated nodes by undoing the node and edge eliminations in reverse order.
When undoing a node elimination for node $w$, \Sys selects the configuration that minimizes Equation~\ref{eqn2} for node $w$. After undoing all eliminations, \Sys has a configuration
for every node in the original graph. In Appendix~\ref{subsec:elimination}, we prove that our algorithm finds an optimal global configuration.
%Our algorithm is able to find a global configuration that minimizes the $\er{Cost}$ function in linear time (proof in Appendix~\ref{subsec:complexity}).
In our experiments, \Sys finds an optimal configuration for parallelizing the largest CNN we have worked with, \inception, on 16 GPUs in about 100ms.


